I Can Find You in Seconds! Leveraging Large Language Models for Code Authorship Attribution

Source code authorship attribution is important in software forensics, plagiarism detection, and protecting software patch integrity. Existing techniques often rely on supervised machine learning, which struggles with generalization across different programming languages and coding styles due to the need for large labeled datasets. Inspired by recent advances in natural language authorship analysis using large language models (LLMs), which have shown exceptional performance without task-specific tuning, this paper explores the use of LLMs for source code authorship attribution. We present a comprehensive study demonstrating that state-of-the-art LLMs can successfully attribute source code authorship across different languages. LLMs can determine whether two code snippets are written by the same author with zero-shot prompting, achieving a Matthews Correlation Coefficient (MCC) of 0.78, and can attribute code authorship from a small set of reference code snippets via few-shot learning, achieving MCC of 0.77. Additionally, LLMs show some adversarial robustness against misattribution attacks. Despite these capabilities, we found that naive prompting of LLMs does not scale well with a large number of authors due to input token limitations. To address this, we propose a tournament-style approach for large-scale attribution. Evaluating this approach on datasets of C++ (500 authors, 26,355 samples) and Java (686 authors, 55,267 samples) code from GitHub, we achieve classification accuracy of up to 65% for C++ and 68.7% for Java using only one reference per author. These results open new possibilities for applying LLMs to code authorship attribution in cybersecurity and software engineering.

==> tables/rq2-one-shot-results.tex <==
\begin{table*}[t]
\begin{minipage}{.47\textwidth}
% Config the row spacing
\def\arraystretch{1.05}
% Config the column spacing
\setlength{\tabcolsep}{2pt}
    \centering
        \caption{Confusion matrix for LLM-based code authorship attribution with one-shot prompts over 200 randomly sampled C++ code samples. () is \# of references.}
        \label{tab:oneshot-cpp-confusion-matrix}
            \begin{tabular}{lcccccccccccccc}
            \Xhline{2\arrayrulewidth}
            \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{P1}}} & \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{P2}}} & \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{P3}}}  \\ \hhline{~----~----~----} 
            \ccd{\textbf{Models}}    & \ccd{\textbf{TP}}  & \ccd{\textbf{FN}}  & \ccd{\textbf{TN}}  & \ccd{\textbf{FP}} &\ccd{} & \ccd{\textbf{TP}}  & \ccd{\textbf{FN}}  & \ccd{\textbf{TN}}  & \ccd{\textbf{FP}} & \ccd{} & \ccd{\textbf{TP}}  & \ccd{\textbf{FN}}  & \ccd{\textbf{TN}}  & \ccd{\textbf{FP}} \\ \Xhline{2\arrayrulewidth}
            Gemini-1.5-p (3)           &      70 &       30 &     94 &       6 &      &      86 &      14 &      85 &      15 &       &      69 &      31 &      95 &     5 \\ 
            \cc{Gemini-1.5-p (5)}      & \cc{70} & \cc{30}  & \cc{93}& \cc{7}  &\cc{} & \cc{82} & \cc{18} & \cc{74} & \cc{26} & \cc{} & \cc{61} & \cc{39} & \cc{95} & \cc{5} \\
            Gemini-1.5-p (7)           &      61 &       39 &     95 &       5 &      &      80 &      20 &      78 &      22 &       &      63 &      37 &       94 &     6 \\   
            \cc{Gemini-1.5-p (10)}     & \cc{62} & \cc{38} & \cc{97} & \cc{3} &\cc{} & \cc{77} & \cc{23} & \cc{83} & \cc{17} & \cc{} & \cc{61} & \cc{39} & \cc{96} & \cc{4} \\
            \Xhline{2\arrayrulewidth}
            GPT-4o (3)                   &      80 &      20 &      62 &       38 &      &      96 &       4 &      23 &       77 &       &      92 &       8 &      28 &      72 \\   
            \cc{GPT-4o (5)}              & \cc{69} & \cc{31} & \cc{72} &  \cc{28} &\cc{} & \cc{83} & \cc{17} & \cc{33} &  \cc{67} & \cc{} & \cc{82} & \cc{18} & \cc{36} & \cc{64} \\
            GPT-4o (7)                   &      62 &      38 &      78 &       22 &      &      77 &      23 &      49 &       51 &       &      79 &      21 &      53 &      57 \\   
            \cc{GPT-4o (10)}             & \cc{54} & \cc{46} & \cc{85} &  \cc{15} &\cc{} & \cc{67} & \cc{33} & \cc{61} &  \cc{39} & \cc{} & \cc{71} & \cc{29} & \cc{67} & \cc{33} \\
            \Xhline{2\arrayrulewidth}
            \end{tabular}
\end{minipage}
%\end{table}
~
~
%\begin{table}[t]
\begin{minipage}{.49\textwidth}
% Config the row spacing
\def\arraystretch{1.05}
% Config the column spacing
\setlength{\tabcolsep}{2pt}
    \centering
        \caption{Accuracy and MCC scores of LLM-based C++ code authorship attribution with one-shot prompts (results of the top accuracy and MCC are shown in \textbf{bold}). () is \# of references.}
        \label{tab:oneshot-cpp-accuracy-mcc}
            \begin{tabular}{lccccccccc}
            \Xhline{2\arrayrulewidth}
            \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{Accuracy(\%)}}} & \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{MCC Scores}}} \\ \hhline{~----~----} 
            \ccd{\textbf{Models}} & \ccd{\textbf{P1}} & \ccd{\textbf{P2}} & \ccd{\textbf{P3}} & \ccd{\textbf{Average}} & \ccd{} & \ccd{\textbf{P1}} & \ccd{\textbf{P2}} & \ccd{\textbf{P3}} & \ccd{\textbf{Average}} \\ \Xhline{2\arrayrulewidth}
            Gemini-1.5-p (3)           & 82.0               & \textbf{85.5}      & 82.0               & 83.2               &       & 0.66              & \textbf{0.71}     & 0.66               & 0.68 \\ 
            \cc{Gemini-1.5-p (5)}      & \cc{81.5}          & \cc{78.0}          & \cc{78.0}          & \cc{79.2}          & \cc{} & \cc{0.65}         & \cc{0.56}         & \cc{0.60}          & \cc{0.60} \\
            Gemini-1.5-p (7)           & 78.0               & 79.0               & 78.5               & 78.5               &       & 0.60              & 0.58              & 0.60               & 0.59 \\
            \cc{Gemini-1.5-p (10)}     & \cc{79.5}          & \cc{80.0}          & \cc{78.5}          & \cc{79.3}          & \cc{} & \cc{0.63}         & \cc{0.60}         & \cc{0.61}          & \cc{0.61} \\
            \Xhline{2\arrayrulewidth}
            GPT-4o (3)                   & \textbf{71.0}      & 59.5               & 60.0               & 63.5               &       & \textbf{0.43}     & 0.28              & 0.26               & 0.32 \\
            \cc{GPT-4o (5)}              & \cc{70.5}          & \cc{58.0}          & \cc{59.0}          & \cc{62.5}          & \cc{} & \cc{0.41}         & \cc{0.18}         & \cc{0.20}          & \cc{0.27} \\
            GPT-4o (7)                   & 70.0               & 63.0               & 66.0               & 66.3               &       & 0.41              & 0.27              & 0.33               & 0.34     \\
            \cc{GPT-4o (10)}             & \cc{69.5}          & \cc{64.0}          & \cc{69.0}          & \cc{67.5}          & \cc{} & \cc{0.41}         & \cc{0.28}         & \cc{0.38}          & \cc{0.36} \\
            \Xhline{2\arrayrulewidth}
            \end{tabular}
\end{minipage}
\end{table*}


% \begin{table*}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{One-Shot: In-Distribution Experiment for C++.}    \label{tab:oneshot-ID-c++}
%             \begin{tabular}{lccc}
%             \Xhline{2\arrayrulewidth}
%             \ccd{Models}                       & \multicolumn{3}{c}{\ccd{\# of correct answers}} \\
%             \ccd{() is \# of references }       & \ccd{P1}              & \ccd{P2}                & \ccd{P3}                     \\
%             \Xhline{2\arrayrulewidth}
%             Gemini-1.5-p (3)              & 70                & 86                    & 69                                             \\
%             \cc{Gemini-1.5-p (5)}         & \cc{70}           & \cc{82}               & \cc{61}                                  \\
%             Gemini-1.5-p (7)              & 61                & 80                    & 63                                             \\
%             \cc{Gemini-1.5-p (10)}        & \cc{62}           & \cc{77}               & \cc{61}                                    \\
%             \Xhline{2\arrayrulewidth}
%             ChatGPT-4o (3)              & 80                & 96                    & 92                                             \\
%             \cc{ChatGPT-4o (5)}         & \cc{69}           & \cc{83}               & \cc{82}                                  \\
%             ChatGPT-4o (7)              & 62                & 77                    & 79                                             \\
%             \cc{ChatGPT-4o (10)}        & \cc{54}           & \cc{67}               & \cc{71}                                    \\
%              \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{minipage}
% %\end{table}
% ~
% %\begin{table}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{One-Shot: Out-Of-Distribution Experiment for C++.}    \label{tab:oneshot-OOD-c++}
%             \begin{tabular}{lccc}
%             \Xhline{2\arrayrulewidth}
%              \ccd{Models}                       & \multicolumn{3}{c}{\ccd{\# of correct answers}} \\
%             \ccd{() is \# of references }       & \ccd{P1}              & \ccd{P2}                & \ccd{P3}                     \\
%             \Xhline{2\arrayrulewidth}
%             Gemini-1.5-p (3)              & 94                & 85                    & 95                                            \\
%             \cc{Gemini-1.5-p (5)}         & \cc{93}           & \cc{74}               & \cc{95}                                  \\
%             Gemini-1.5-p (7)              & 95                & 78                    & 94                                             \\
%             \cc{Gemini-1.5-p (10)}        & \cc{97}           & \cc{83}               & \cc{96}                                    \\
%             \Xhline{2\arrayrulewidth}
%             ChatGPT-4o (3)              & 62                & 23                    & 28                                             \\
%             \cc{ChatGPT-4o (5)}         & \cc{72}           & \cc{33}               & \cc{36}                                  \\
%             ChatGPT-4o (7)              & 78                & 49                    & 53                                             \\
%             \cc{ChatGPT-4o (10)}        & \cc{85}           & \cc{61}               & \cc{67}                                    \\
%              \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{minipage}
% %\end{table}
% ~
% %\begin{table}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{One-Shot: MCC Scores for C++.}    \label{tab:oneshot-MCC-c++}
%             \begin{tabular}{lcccc}
%             \Xhline{2\arrayrulewidth}
%              \ccd{\multirow{2}{*}{Models}} & \multicolumn{4}{c}{\ccd{\begin{tabular}[c]{@{}c@{}} MCC \\ Scores \end{tabular}}} \\
%             \ccd{ }                             & \ccd{P1}                  & \ccd{P2}                 & \ccd{P3}     & \ccd{\textbf{Average}}            \\
%             \Xhline{2\arrayrulewidth}
%             Gemini-1.5-p (3)              & 0.66              & \textbf{0.71}           & 0.66                & \textbf{0.68}           \\
%             \cc{Gemini-1.5-p (5)}         & \cc{0.65}         & \cc{0.56}               & \cc{0.60}           & \cc{0.60}          \\
%             Gemini-1.5-p (7)              & 0.60              & 0.58                    & 0.60                & 0.59           \\
%             \cc{Gemini-1.5-p (10)}        & \cc{0.63}         & \cc{0.60}               & \cc{0.61}           & \cc{0.61}            \\
%             \Xhline{2\arrayrulewidth}
%             \textbf{Average}                & \textbf{0.63}     & 0.61                    & 0.62                &             \\
%             \Xhline{2\arrayrulewidth}
%             ChatGPT-4o (3)              &\textbf{0.43}        & 0.28                    & 0.26                  & 0.32                           \\
%             \cc{ChatGPT-4o (5)}         & \cc{0.41}           & \cc{0.18}               & \cc{0.20}             & \cc{0.27}                     \\
%             ChatGPT-4o (7)              & 0.41                & 0.27                    & 0.33                  & 0.34                           \\
%             \cc{ChatGPT-4o (10)}        & \cc{0.41}           & \cc{0.28}                & \cc{0.38}             & \textbf{\cc{0.36}}                       \\
%              \Xhline{2\arrayrulewidth}
%              \textbf{Average}              & \textbf{0.41}    & 0.25                    & 0.29                  &             \\
%             \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{minipage}
% \end{table*}




==> tables/rq2-three-shot-results.tex <==

\begin{table*}[t]
\begin{minipage}{.47\textwidth}
% Config the row spacing
\def\arraystretch{1.05}
% Config the column spacing
\setlength{\tabcolsep}{2pt}
    \centering
        \caption{Confusion matrix for LLM-based code authorship attribution with three-shot prompts over 200 randomly sampled C++ code samples. () is \# of references.}
        \label{tab:threeshot-cpp-confusion-matrix}
            \begin{tabular}{lcccccccccccccc}
            \Xhline{2\arrayrulewidth}
            \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{P1}}} & \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{P2}}} & \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{P3}}}  \\ \hhline{~----~----~----} 
            \ccd{\textbf{Models}}    & \ccd{\textbf{TP}}  & \ccd{\textbf{FN}}  & \ccd{\textbf{TN}}  & \ccd{\textbf{FP}} &\ccd{} & \ccd{\textbf{TP}}  & \ccd{\textbf{FN}}  & \ccd{\textbf{TN}}  & \ccd{\textbf{FP}} & \ccd{} & \ccd{\textbf{TP}}  & \ccd{\textbf{FN}}  & \ccd{\textbf{TN}}  & \ccd{\textbf{FP}} \\ \Xhline{2\arrayrulewidth}
            Gemini-1.5-p (3)           &      97 &       3 &     72 &       28 &      &      98 &      2 &      57 &      43 &       &      97 &      3 &      77 &     23 \\ 
            \cc{Gemini-1.5-p (5)}      & \cc{90} & \cc{10} & \cc{71}&  \cc{29} &\cc{} & \cc{98} & \cc{2} & \cc{63} & \cc{37} & \cc{} & \cc{93} & \cc{7} & \cc{75} & \cc{25} \\
            Gemini-1.5-p (7)           &      92 &       8 &     76 &       24 &      &      95 &      5 &      58 &      42 &       &      89 &     11 &      68 &     32 \\   
            \Xhline{2\arrayrulewidth}
            \cc{GPT-4o (3)}              & \cc{96} & \cc{4}  & \cc{37} &  \cc{63} &\cc{} & \cc{98} & \cc{2} & \cc{11} &  \cc{89} & \cc{} & \cc{98} & \cc{2} & \cc{17} & \cc{83} \\
            GPT-4o (5)                   &      87 &      13 &      42 &       58 &      &      91 &       9 &      31 &       69 &       &      93 &       7 &      27 &      73 \\   
            \cc{GPT-4o (7)}              & \cc{77} & \cc{23} & \cc{49} &  \cc{51} &\cc{} & \cc{85} & \cc{15} & \cc{34} &  \cc{6} & \cc{} & \cc{90} & \cc{10} & \cc{27} & \cc{73} \\
            \Xhline{2\arrayrulewidth}
            \end{tabular}
\end{minipage}
%\end{table}
~
~
%\begin{table}[t]
\begin{minipage}{.49\textwidth}
% Config the row spacing
\def\arraystretch{1.05}
% Config the column spacing
\setlength{\tabcolsep}{2pt}
    \centering
        \caption{Accuracy and MCC scores of LLM-based C++ code authorship attribution with three-shot prompts (results of the top accuracy and MCC are shown in \textbf{bold}). () is \# of references.}
        \label{tab:threeshot-cpp-accuracy-mcc}
            \begin{tabular}{lccccccccc}
            \Xhline{2\arrayrulewidth}
            \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{Accuracy(\%)}}} & \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{MCC Scores}}} \\ \hhline{~----~----} 
            \ccd{\textbf{Models}} & \ccd{\textbf{P1}} & \ccd{\textbf{P2}} & \ccd{\textbf{P3}} & \ccd{\textbf{Average}} & \ccd{} & \ccd{\textbf{P1}} & \ccd{\textbf{P2}} & \ccd{\textbf{P3}} & \ccd{\textbf{Average}} \\ \Xhline{2\arrayrulewidth}
            Gemini-1.5-p (3)           & 84.5                & 77.5               & \textbf{87.0}      & 83.0               &       & 0.71               & 0.60              & \textbf{0.76}      & 0.69 \\ 
            \cc{Gemini-1.5-p (5)}      & \cc{80.5}           & \cc{80.5}          & \cc{84.0}          & \cc{81.7}          & \cc{} & \cc{0.62}          & \cc{0.65}         & \cc{0.69}          & \cc{0.65} \\
            Gemini-1.5-p (7)           & 84.0                & 76.5               & 78.5               & 79.7               &       & 0.69               & 0.57              & 0.58               & 0.61 \\
            \Xhline{2\arrayrulewidth}
            \cc{GPT-4o (3)}              & \cc{\textbf{66.5}}  & \cc{54.5}          & \cc{57.5}          & \cc{59.5}          & \cc{} & \cc{\textbf{0.41}} & \cc{0.18}         & \cc{0.26}          & \cc{0.28} \\
            GPT-4o (5)                   & 64.5                & 61.0               & 60.0               & 61.8               &       & 0.32               & 0.28              & 0.27               & 0.29 \\
            \cc{GPT-4o (7)}              & \cc{63.0}           & \cc{59.5}          & \cc{58.5}          & \cc{60.3}          & \cc{} & \cc{0.27}          & \cc{0.22}         & \cc{0.22}          & \cc{0.24} \\            \Xhline{2\arrayrulewidth}
            \end{tabular}
\end{minipage}
\end{table*}



% \begin{table*}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{Three-Shot: In-Distribution Experiment for C++.}    \label{tab:Threeshot-ID-c++}
%             \begin{tabular}{lccc}
%             \Xhline{2\arrayrulewidth}
%              \ccd{Models}                       & \multicolumn{3}{c}{\ccd{\# of correct answers}} \\
%             \ccd{() is \# of references }       & \ccd{P1}              & \ccd{P2}                & \ccd{P3}                     \\
%             \Xhline{2\arrayrulewidth}
%             Gemini-1.5-p (3)             & 97                    & 98                      & 97                       \\
%             \cc{Gemini-1.5-p (5)}        & \cc{90}               & \cc{98}                 & \cc{93}                 \\
%             Gemini-1.5-p (7)             & 91                    & 95                      & 89                       \\
%             \Xhline{2\arrayrulewidth}
%             \cc{ChatGPT-4o (3)}         & \cc{96}           & \cc{98}               & \cc{98}                                  \\
%             ChatGPT-4o (5)              & 87                & 91                    & 93                                             \\
%             \cc{ChatGPT-4o (7)}         & \cc{77}           & \cc{85}               & \cc{90}                                  \\
%             \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{minipage}
% %\end{table}
% ~
% %\begin{table}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{Three-Shot: Out-Of-Distribution Experiment for C++.}    \label{tab:Threeshot-OOD-c++}
%             \begin{tabular}{lccc}
%             \Xhline{2\arrayrulewidth}
%              \ccd{Models}                       & \multicolumn{3}{c}{\ccd{\# of correct answers}} \\
%             \ccd{() is \# of references }       & \ccd{P1}              & \ccd{P2}                & \ccd{P3}                     \\
%             \Xhline{2\arrayrulewidth}
%             Gemini-1.5-p (3)              & 72                    & 57                      & 77                       \\
%             \cc{Gemini-1.5-p (5)}         & \cc{72}               & \cc{63}                 & \cc{75}                 \\
%             Gemini-1.5-p (7)              & 76                    & 58                      & 68                       \\
%             \Xhline{2\arrayrulewidth}
%             \cc{ChatGPT-4o (3)}         & \cc{37}           & \cc{11}               & \cc{17}                                  \\
%             ChatGPT-4o (5)              & 42                & 31                    & 27                                             \\
%             \cc{ChatGPT-4o (7)}         & \cc{49}           & \cc{34}               & \cc{27}                                  \\
%             \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{minipage}
% %\end{table}
% ~
% %\begin{table}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{Three-Shot: MCC Scores for C++.}    \label{tab:Threeshot-MCC-c++}
%             \begin{tabular}{lcccc}
%             \Xhline{2\arrayrulewidth}
%              \ccd{\multirow{2}{*}{Models}} & \multicolumn{4}{c}{\ccd{\begin{tabular}[c]{@{}c@{}} MCC \\ Scores \end{tabular}}} \\
%             \ccd{ }                             & \ccd{P1}                  & \ccd{P2}                 & \ccd{P3}           & \ccd{\textbf{Average}}     \\
%             \Xhline{2\arrayrulewidth}
%             Gemini-1.5-p (3)              & 0.71                    & 0.60                    & \textbf{0.76}       & \textbf{0.69}       \\
%             \cc{Gemini-1.5-p (5)}         & \cc{0.62}               & \cc{0.65}               & \cc{0.69}           & \cc{0.65}       \\
%             Gemini-1.5-p (7)              & 0.69                    & 0.57                    & 0.58                & 0.61        \\
%             \Xhline{2\arrayrulewidth}
%             \cc{\textbf{Average}}           & \cc{0.67}               & \cc{0.61}               & \cc{\textbf{0.68}}           &  \cc{}                        \\
%             \Xhline{2\arrayrulewidth}
%             ChatGPT-4o (3)              & \textbf{0.41}           & 0.18                    & 0.26       & 0.28       \\
%             \cc{ChatGPT-4o (5)}         & \cc{0.32}               & \cc{0.28}               & \cc{0.27}           & \textbf{\cc{0.29}}       \\
%             ChatGPT-4o (7)              & 0.27                    & 0.22                    & 0.22                & 0.24        \\
%             \Xhline{2\arrayrulewidth}
%             \cc{\textbf{Average}}           & \cc{\textbf{0.33}}       & \cc{0.25}               & \cc{0.25}           &  \cc{}                        \\
%             \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{minipage}
% \end{table*}


==> tables/rq2-two-shot-results.tex <==
\begin{table*}[t]
\begin{minipage}{.47\textwidth}
% Config the row spacing
\def\arraystretch{1.05}
% Config the column spacing
\setlength{\tabcolsep}{2pt}
    \centering
        \caption{Confusion matrix for LLM-based code authorship attribution with two-shot prompts over 200 randomly sampled C++ code samples. () is \# of references.}
        \label{tab:twoshot-cpp-confusion-matrix}
            \begin{tabular}{lcccccccccccccc}
            \Xhline{2\arrayrulewidth}
            \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{P1}}} & \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{P2}}} & \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{P3}}}  \\ \hhline{~----~----~----} 
            \ccd{\textbf{Models}}    & \ccd{\textbf{TP}}  & \ccd{\textbf{FN}}  & \ccd{\textbf{TN}}  & \ccd{\textbf{FP}} &\ccd{} & \ccd{\textbf{TP}}  & \ccd{\textbf{FN}}  & \ccd{\textbf{TN}}  & \ccd{\textbf{FP}} & \ccd{} & \ccd{\textbf{TP}}  & \ccd{\textbf{FN}}  & \ccd{\textbf{TN}}  & \ccd{\textbf{FP}} \\ \Xhline{2\arrayrulewidth}
            Gemini-1.5-p (3)           &      91 &       9 &     86  &       14 &      &      99 &      1  &      63 &      37 &       &      93 &      7  &      78 &     22 \\ 
            \cc{Gemini-1.5-p (5)}      & \cc{87} & \cc{13} & \cc{83} & \cc{17}  &\cc{} & \cc{96} & \cc{4}  & \cc{66} & \cc{34} & \cc{} & \cc{85} & \cc{15} & \cc{83} & \cc{17} \\
            Gemini-1.5-p (7)           &      88 &       12 &     87 &      13  &      &      95 &      5  &      68 &      32 &       &      84 &      16 &      82 &     18 \\   
            \cc{Gemini-1.5-p (10)}     & \cc{78} & \cc{22} & \cc{79} & \cc{21}  &\cc{} & \cc{87} & \cc{13} & \cc{66} & \cc{34} & \cc{} & \cc{83} & \cc{17} & \cc{84} & \cc{16} \\
            \Xhline{2\arrayrulewidth}
            GPT-4o (3)                   &      95 &      5  &      34 &       66 &      &      95 &       5 &      12 &       88 &       &      96 &       4 &      12 &      88 \\   
            \cc{GPT-4o (5)}              & \cc{85} & \cc{15} & \cc{49} &  \cc{51} &\cc{} & \cc{92} & \cc{8}  & \cc{25} &  \cc{75} & \cc{} & \cc{97} & \cc{3} & \cc{25} & \cc{75} \\
            GPT-4o (7)                   &      81 &      19 &      62 &       38 &      &      88 &      12 &      36 &       64 &       &      85 &      15 &      39 &      61 \\   
            \cc{GPT-4o (10)}             & \cc{65} & \cc{35} & \cc{62} &  \cc{38} &\cc{} & \cc{76} & \cc{24} & \cc{40} &  \cc{60} & \cc{} & \cc{75} & \cc{25} & \cc{49} & \cc{51} \\
            \Xhline{2\arrayrulewidth}
            \end{tabular}
\end{minipage}
%\end{table}
~
~
%\begin{table}[t]
\begin{minipage}{.49\textwidth}
% Config the row spacing
\def\arraystretch{1.05}
% Config the column spacing
\setlength{\tabcolsep}{2pt}
    \centering
        \caption{Accuracy and MCC scores of LLM-based C++ code authorship attribution with two-shot prompts (results of the top accuracy and MCC are shown in \textbf{bold}). () is \# of references.}
        \label{tab:twoshot-cpp-accuracy-mcc}
            \begin{tabular}{lccccccccc}
            \Xhline{2\arrayrulewidth}
            \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{Accuracy(\%)}}} & \ccd{} & \multicolumn{4}{c}{\ccd{\textbf{MCC Scores}}} \\ \hhline{~----~----} 
            \ccd{\textbf{Models}} & \ccd{\textbf{P1}} & \ccd{\textbf{P2}} & \ccd{\textbf{P3}} & \ccd{\textbf{Average}} & \ccd{} & \ccd{\textbf{P1}} & \ccd{\textbf{P2}} & \ccd{\textbf{P3}} & \ccd{\textbf{Average}} \\ \Xhline{2\arrayrulewidth}
            Gemini-1.5-p (3)           & \textbf{88.5}      & 81.0               & 85.5               & 85.0               &       & \textbf{0.77}              & 0.66     & 0.72               & 0.72 \\ 
            \cc{Gemini-1.5-p (5)}      & \cc{85.0}          & \cc{81.0}          & \cc{84.0}          & \cc{83.3}          & \cc{} & \cc{0.70}         & \cc{0.65}         & \cc{0.68}          & \cc{0.68} \\
            Gemini-1.5-p (7)           & 87.5               & 81.5               & 83.0               & 84.0               &       & 0.75              & 0.65              & 0.66               & 0.69 \\
            \cc{Gemini-1.5-p (10)}     & \cc{78.5}          & \cc{76.5}          & \cc{83.5}          & \cc{79.5}          & \cc{} & \cc{0.57}         & \cc{0.54}         & \cc{0.67}          & \cc{0.59} \\
            \Xhline{2\arrayrulewidth}
            GPT-4o (3)                   & 64.5               & 53.5               & 54.0               & 57.3               &       & 0.37              & 0.13              & 0.15               & 0.21 \\
            \cc{GPT-4o (5)}              & \cc{67.0}          & \cc{58.5}          & \cc{61.0}          & \cc{62.2}          & \cc{} & \cc{0.36}         & \cc{0.23}         & \cc{0.32}          & \cc{0.30} \\
            GPT-4o (7)                   & \textbf{71.5}      & 62.0               & 62.0               & 65.2               &       & \textbf{0.44}     & 0.28              & 0.27               & 0.33      \\
            \cc{GPT-4o (10)}             & \cc{63.5}          & \cc{58.0}          & \cc{62.0}          & \cc{61.2}          & \cc{} & \cc{0.27}         & \cc{0.17}         & \cc{0.25}          & \cc{0.23} \\
            \Xhline{2\arrayrulewidth}
            \end{tabular}
\end{minipage}
\end{table*}


% \begin{table*}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{Two-Shot: In-Distribution Experiment for C++.}    \label{tab:Twoshot-ID-c++}
%             \begin{tabular}{lccc}
%             \Xhline{2\arrayrulewidth}
%              \ccd{Models}                       & \multicolumn{3}{c}{\ccd{\# of correct answers}} \\
%             \ccd{() is \# of references }       & \ccd{P1}              & \ccd{P2}                & \ccd{P3}                     \\
%             \Xhline{2\arrayrulewidth}
%             Gemini-1.5-p (3)              & 91                 & 99                    & 93                                             \\
%             \cc{Gemini-1.5-p (5)}         & \cc{87}            & \cc{96}               & \cc{85}                                  \\
%             Gemini-1.5-p (7)              & 88                 & 95                    & 84                                          \\
%             \cc{Gemini-1.5-p (10)}        & \cc{78}            & \cc{87}               & \cc{83}                                  \\
%             \Xhline{2\arrayrulewidth}
%             ChatGPT-4o (3)              & 95                & 95                    & 96                                             \\
%             \cc{ChatGPT-4o (5)}         & \cc{85}           & \cc{92}               & \cc{97}                                  \\
%             ChatGPT-4o (7)              & 81                & 88                    & 85                                             \\
%             \cc{ChatGPT-4o (10)}        & \cc{65}           & \cc{76}               & \cc{75}                                    \\
%              \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{minipage}
% %\end{table}
% ~
% %\begin{table}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{Two-Shot: Out-Of-Distribution Experiment for C++.}    \label{tab:Twoshot-OOD-c++}
%             \begin{tabular}{lccc}
%             \Xhline{2\arrayrulewidth}
%              \ccd{Models}                       & \multicolumn{3}{c}{\ccd{\# of correct answers}} \\
%             \ccd{() is \# of references }       & \ccd{P1}              & \ccd{P2}                & \ccd{P3}                     \\
%             \Xhline{2\arrayrulewidth}
%             Gemini-1.5-p (3)              & 86                    & 63                    & 78                                             \\
%             \cc{Gemini-1.5-p (5)}         & \cc{83}               & \cc{66}               & \cc{83}                                  \\
%             Gemini-1.5-p (7)              & 87                    & 68                    & 82                                            \\
%             \cc{Gemini-1.5-p (10)}        & \cc{79}               & \cc{66}               & \cc{84}                                  \\
%             \Xhline{2\arrayrulewidth}
%             ChatGPT-4o (3)              & 34                & 12                    & 12                                             \\
%             \cc{ChatGPT-4o (5)}         & \cc{49}           & \cc{25}               & \cc{25}                                  \\
%             ChatGPT-4o (7)              & 62                & 36                    & 39                                             \\
%             \cc{ChatGPT-4o (10)}        & \cc{62}           & \cc{40}               & \cc{49}                                    \\
%              \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{minipage}
% %\end{table}
% ~
% %\begin{table}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{Two-Shot: MCC Scores for C++.}    \label{tab:Twoshot-MCC-c++}
%             \begin{tabular}{lcccc}
%             \Xhline{2\arrayrulewidth}
%              \ccd{\multirow{2}{*}{Models}} & \multicolumn{4}{c}{\ccd{\begin{tabular}[c]{@{}c@{}} MCC \\ Scores \end{tabular}}} \\
%             \ccd{ }                             & \ccd{P1}                  & \ccd{P2}                 & \ccd{P3}         & \ccd{\textbf{Average}}       \\
%             \Xhline{2\arrayrulewidth}
%             Gemini-1.5-p (3)              & \textbf{0.77}         & 0.66                    & 0.72                    & \textbf{0.72}                         \\
%             \cc{Gemini-1.5-p (5)}         & \cc{0.70}             & \cc{0.65}               & \cc{0.68}               & \cc{0.68}                   \\
%             Gemini-1.5-p (7)              & 0.75                  & 0.65                    & 0.66                    & 0.69                         \\
%             \cc{Gemini-1.5-p (10)}        & \cc{0.57}             & \cc{0.56}               & \cc{0.67}               & \cc{0.59}                    \\
%             \Xhline{2\arrayrulewidth}
%             \textbf{Average}                   & \textbf{0.70}         & 0.63                    & 0.68                    &                          \\
%             \Xhline{2\arrayrulewidth}
%             ChatGPT-4o (3)              & 0.37                & 0.13                    & 0.15                  & 0.21                           \\
%             \cc{ChatGPT-4o (5)}         & \cc{0.36}           & \cc{0.23}               & \cc{0.32}             & \cc{0.30}                     \\
%             ChatGPT-4o (7)              & \textbf{0.44}                & 0.28                    & 0.27         & \textbf{0.33}                           \\
%             \cc{ChatGPT-4o (10)}        & \cc{0.27}           & \cc{0.17}               & \cc{0.25}             & \cc{0.23}                       \\
%              \Xhline{2\arrayrulewidth}
%              \textbf{Average}           & \textbf{0.36}        & 0.20                    & 0.25               &             \\
%             \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{minipage}
% \end{table*}

==> tables/rq5-java-three-shot-results.tex <==
\begin{table}[t]
% \begin{minipage}{.47\textwidth}
% Config the row spacing
\def\arraystretch{1.05}
% Config the column spacing
\setlength{\tabcolsep}{2pt}
    \centering
        \caption{Confusion matrix, Accuracy, and MCC scores for LLM-based code authorship attribution with three-shot prompt (P1 only) over 200 randomly sampled Java code samples (results of the top accuracy and MCC are shown in \textbf{bold}). () is \# of references.}
        \label{tab:zeroshot-cpp-confusion-matrix}
            \begin{tabular}{lcccc|cccc}
            \Xhline{2\arrayrulewidth}
            \ccd{\textbf{Models}}    & \ccd{\textbf{TP}}  & \ccd{\textbf{FP}}  & \ccd{\textbf{TN}}  & \ccd{\textbf{FN}} & \ccd{\textbf{Accuracy(\%)}} & \ccd{\textbf{MCC Scores}} \\ \Xhline{2\arrayrulewidth}
            Gemini-1.5-pro (3)          &      98 &      2  &      61 &      39   & \textbf{79.5}  & \textbf{0.64}      \\   
            \cc{Gemini-1.5-pro (5)}     & \cc{100} & \cc{0}  & \cc{48} &  \cc{52}  & \cc{74.0}      & \cc{0.56}    \\
            \Xhline{2\arrayrulewidth}
            GPT-4o (3)                  &      100 &      0 &      17 &      83   & \textbf{58.5}   & \textbf{0.30}      \\   
            \cc{GPT-4o (5)}             & \cc{100} & \cc{0} & \cc{18}  &  \cc{82}  & \cc{59.0}       & \cc{0.31}    \\
            \Xhline{2\arrayrulewidth}
            \end{tabular}
% \end{minipage}
\end{table}



% \begin{table}[t]
%     \centering
%         \caption{Three-Shot: Experiment for Java with P1 only.}    \label{tab:Threeshot-Java}
%             \begin{tabular}{lccc}
%             \Xhline{2\arrayrulewidth}
%             \multicolumn{1}{c}{\multirow{2}{*}{\ccd{}}} & \multicolumn{2}{l}{\ccd{\# of correct answers}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\ccd{MCC} \\ \ccd{Score} \end{tabular}} \\
%             \multicolumn{1}{c}{\ccd{Models}}                        & \ccd{ID}              & \ccd{OOD}             &    \ccd{}      \\
%             \Xhline{2\arrayrulewidth}
%             Gemini-1.5-pro (3)                  & 98                        & 61                        & \bf{0.64}                                          \\            
%             \cc{Gemini-1.5-pro (5)}                 & \cc{100}                  & \cc{48}                  & \cc{0.56}                                        \\
%             \Xhline{2\arrayrulewidth}
%             Average                             &                              &                               & 0.60 \\
%             \Xhline{2\arrayrulewidth}           
%             \cc{ChatGPT-4o (3)}                   & \cc{100}                        & \cc{17}                & \cc{0.30}                                         \\
%             ChatGPT-4o (5)                     & 100                  & 18                  & \bf{0.31}                               \\
%             \Xhline{2\arrayrulewidth}
%             \cc{Average}                             &     \cc{}                          &       \cc{}                        & \cc{0.31} \\
%             \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{table}


% \begin{table*}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{Three-Shot: In-Distribution Experiment for Java}    \label{tab:Threeshot-ID-Java}
%             \begin{tabular}{lccc}
%             \Xhline{2\arrayrulewidth}
%             \ccd{Models}                       & \multicolumn{3}{c}{\ccd{\# of correct answers}} \\
%             \ccd{() is \# of references }       & \ccd{P1}              & \ccd{P2}                & \ccd{P3}                     \\
%             \Xhline{2\arrayrulewidth}                                    
%             Gemini-1.5-pro (3)              & 98                & 98                    & 99                                             \\
%             \cc{Gemini-1.5-pro (5)}         & \cc{-}           & \cc{-}               & \cc{-}                                  \\
%             \Xhline{2\arrayrulewidth}
%             ChatGPT-4o (3)              & 100                & -                    & -                                             \\
%             \cc{ChatGPT-4o (5)}         & \cc{100}           & \cc{-}               & \cc{-}                                  \\
%             \Xhline{2\arrayrulewidth}
%             \end{tabular}
% %\end{table}
% \end{minipage}
% ~
% %begin{table}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{Three-Shot: Out-Of-Distribution Experiment for Java}    \label{tab:Threeshot-OOD-Java}
%             \begin{tabular}{lccc}
%             \Xhline{2\arrayrulewidth}
%              \ccd{Models}                       & \multicolumn{3}{c}{\ccd{\# of correct answers}} \\
%             \ccd{() is \# of references }       & \ccd{P1}              & \ccd{P2}                & \ccd{P3}                     \\
%             \Xhline{2\arrayrulewidth}                                    
%             Gemini-1.5-pro (3)              & 61                & 42                    & 79                                            \\
%             \cc{Gemini-1.5-pro (5)}         & \cc{-}           & \cc{-}               & \cc{-}                                  \\
%             \Xhline{2\arrayrulewidth}
%             ChatGPT-4o (3)              & 17                & -                    & -                                             \\
%             \cc{ChatGPT-4o (5)}         & \cc{18}           & \cc{-}               & \cc{-}                                  \\
%             \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{minipage}
% %\end{table}
% ~
% %\begin{table}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{Three-Shot: MCC Scores for Java}    \label{tab:Threeshot-MCC-Java}
%             \begin{tabular}{lcccc}
%             \Xhline{2\arrayrulewidth}
%              \ccd{\multirow{2}{*}{Models}} & \multicolumn{4}{c}{\ccd{\begin{tabular}[c]{@{}c@{}} MCC \\ Scores \end{tabular}}} \\
%             \ccd{ }                             & \ccd{P1}                  & \ccd{P2}                 & \ccd{P3}     & \ccd{\textbf{Average}}            \\
%             \Xhline{2\arrayrulewidth}                                    
%             Gemini-1.5-pro (3)              & 0.64              & 0.48                    & \textbf{0.80}                 & \textbf{0.64}           \\
%             \cc{Gemini-1.5-pro (5)}         & \cc{-}         & \cc{0.-}               & \cc{0.-}                     & \cc{-}          \\
%             \Xhline{2\arrayrulewidth}
%             \textbf{Average}                & 0.-              & 0.-                    & \textbf{0.-}                &             \\
%             \Xhline{2\arrayrulewidth}
%             ChatGPT-4o (3)              & 0.30              & -                    & \textbf{-}                 & \textbf{-}           \\
%             \cc{ChatGPT-4o (5)}         & \cc{0.31}         & \cc{-}               & \cc{-}                     & \cc{-}          \\
%             \Xhline{2\arrayrulewidth}
%             \textbf{Average}                & 0.31              & -                    & \textbf{-}                &             \\
%             \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{minipage}
% \end{table*}

==> tables/rq5-java-two-shot-results.tex <==
\begin{table}[t]
% \begin{minipage}{.47\textwidth}
% Config the row spacing
\def\arraystretch{1.05}
% Config the column spacing
\setlength{\tabcolsep}{2pt}
    \centering
        \caption{Confusion matrix, Accuracy, and MCC scores for LLM-based code authorship attribution with two-shot prompt (P1 only) over 200 randomly sampled Java code samples (results of the top accuracy and MCC are shown in \textbf{bold}). () is \# of references.}
        \label{tab:zeroshot-cpp-confusion-matrix}
            \begin{tabular}{lcccc|cccc}
            \Xhline{2\arrayrulewidth}
            \ccd{\textbf{Models}}    & \ccd{\textbf{TP}}  & \ccd{\textbf{FP}}  & \ccd{\textbf{TN}}  & \ccd{\textbf{FN}} & \ccd{\textbf{Accuracy(\%)}} & \ccd{\textbf{MCC Scores}} \\ \Xhline{2\arrayrulewidth}
            Gemini-1.5-pro (3)          &      97 &      3  &      62 &      38    & \textbf{79.5}       & \textbf{0.63}      \\   
            \cc{Gemini-1.5-pro (5)}     & \cc{96} & \cc{4}  & \cc{55} &  \cc{45}   & \cc{75.5}           & \cc{0.56}    \\
            Gemini-1.5-pro (7)          &      98 &       2 &     43  &       57   & 70.5                & 0.49      \\   
            \Xhline{2\arrayrulewidth}
            \cc{GPT-4o (3)}             & \cc{100} & \cc{0} & \cc{12}  &  \cc{88}  & \cc{\textbf{56.0}}  & \cc{\textbf{0.25}}    \\
            GPT-4o (5)                  &      100 &      0 &     9  &      91     & 54.5                & 0.22      \\   
            \cc{GPT-4o (7)}            & \cc{100} & \cc{0} & \cc{11} &  \cc{9}     & \cc{55.5}           & \cc{0.24}    \\
            \Xhline{2\arrayrulewidth}
            \end{tabular}
% \end{minipage}
\end{table}


% \begin{table}[t]
%     \centering
%         \caption{Two-Shot: Experiment for Java with P1 only.}    \label{tab:Twoshot-Java}
%             \begin{tabular}{lccc}
%             \Xhline{2\arrayrulewidth}
%             \multicolumn{1}{c}{\multirow{2}{*}{\ccd{}}} & \multicolumn{2}{l}{\ccd{\# of correct answers}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\ccd{MCC} \\ \ccd{Score} \end{tabular}} \\
%             \multicolumn{1}{c}{\ccd{Models}}                        & \ccd{ID}              & \ccd{OOD}             &    \ccd{}      \\
%             \Xhline{2\arrayrulewidth}
%             Gemini-1.5-pro (3)                  & 97                        & 62                        & \bf{0.63}                                          \\            
%             \cc{Gemini-1.5-pro (5)}                 & \cc{96}                  & \cc{55}                  & \cc{0.56}                                        \\
%             Gemini-1.5-pro (7)                   & 98                        & 43                        & 0.49                                         \\
%             \Xhline{2\arrayrulewidth}
%             \cc{Average}                             &     \cc{}                          &      \cc{}                         & \cc{0.56} \\
%             \Xhline{2\arrayrulewidth}           
%             ChatGPT-4o (3)                 & 100                  & 12                  & \bf{0.25}                                        \\
%             \cc{ChatGPT-4o (5)}                   & \cc{100}                        & \cc{9}                & \cc{0.22}                                         \\
%             ChatGPT-4o (7)                     & 100                  & 11                  & 0.24                               \\
%             \Xhline{2\arrayrulewidth}
%             \cc{Average}                             &     \cc{}                          &       \cc{}                        & \cc{0.24} \\
%             \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{table}


% \begin{table*}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{Two-Shot: In-Distribution Experiment for Java}    \label{tab:Twoshot-ID-Java}
%             \begin{tabular}{lccc}
%             \Xhline{2\arrayrulewidth}
%             \ccd{Models}                       & \multicolumn{3}{c}{\ccd{\# of correct answers}} \\
%             \ccd{() is \# of references }       & \ccd{P1}              & \ccd{P2}                & \ccd{P3}                     \\
%             \Xhline{2\arrayrulewidth}                                    
%             Gemini-1.5-pro (3)              & 97                & 98                    & 98                                             \\
%             \cc{Gemini-1.5-pro (5)}         & \cc{96}           & \cc{96}               & \cc{96}                                  \\
%             Gemini-1.5-pro (7)              & 98                & 96                    & 95                                             \\
%             \Xhline{2\arrayrulewidth}
%             \cc{ChatGPT-4o (3)}         & \cc{100}           & \cc{-}               & \cc{-}                                  \\
%             ChatGPT-4o (5)              & 100                & -                    & -                                             \\
%             \cc{ChatGPT-4o (7)}         & \cc{100}           & \cc{-}               & \cc{-}                                  \\
%             \Xhline{2\arrayrulewidth}
%             \end{tabular}
% %\end{table}
% \end{minipage}
% ~
% %begin{table}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{Two-Shot: Out-Of-Distribution Experiment for Java}    \label{tab:Twoshot-OOD-Java}
%             \begin{tabular}{lccc}
%             \Xhline{2\arrayrulewidth}
%              \ccd{Models}                       & \multicolumn{3}{c}{\ccd{\# of correct answers}} \\
%             \ccd{() is \# of references }       & \ccd{P1}              & \ccd{P2}                & \ccd{P3}                     \\
%             \Xhline{2\arrayrulewidth}                                    
%             Gemini-1.5-pro (3)              & 62                & 52                    & 65                                            \\
%             \cc{Gemini-1.5-pro (5)}         & \cc{55}           & \cc{43}               & \cc{58}                                  \\
%             Gemini-1.5-pro (7)              & 43                & 34                    & 52                                             \\
%             \Xhline{2\arrayrulewidth}
%             \cc{ChatGPT-4o (3)}         & \cc{12}           & \cc{-}               & \cc{-}                                  \\
%             ChatGPT-4o (5)              & 9                & -                    & -                                             \\
%             \cc{ChatGPT-4o (7)}         & \cc{11}           & \cc{-}               & \cc{-}                                  \\
%             \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{minipage}
% %\end{table}
% ~
% %\begin{table}[t]
% \begin{minipage}{.3\textwidth}
%     \centering
%         \caption{Two-Shot: MCC Scores for Java}    \label{tab:Twoshot-MCC-Java}
%             \begin{tabular}{lcccc}
%             \Xhline{2\arrayrulewidth}
%              \ccd{\multirow{2}{*}{Models}} & \multicolumn{4}{c}{\ccd{\begin{tabular}[c]{@{}c@{}} MCC \\ Scores \end{tabular}}} \\
%             \ccd{ }                             & \ccd{P1}                  & \ccd{P2}                 & \ccd{P3}     & \ccd{\textbf{Average}}            \\
%             \Xhline{2\arrayrulewidth}                                    
%             Gemini-1.5-pro (3)              & 0.63              & 0.56                    & \textbf{0.67}                 & \textbf{0.62}           \\
%             \cc{Gemini-1.5-pro (5)}         & \cc{0.56}         & \cc{0.46}               & \cc{0.58}                     & \cc{0.53}          \\
%             Gemini-1.5-pro (7)              & 0.49              & 0.38                    & 0.52                           & 0.46           \\
%             \Xhline{2\arrayrulewidth}
%             \cc{\textbf{Average}}           &\cc{0.56}          & \cc{0.47}               & \cc{\textbf{0.59}}                &  \cc{ }           \\
%             \Xhline{2\arrayrulewidth}
%             ChatGPT-4o (3)              & 0.25              & -                    & \textbf{-}                 & \textbf{-}           \\
%             \cc{ChatGPT-4o (5)}         & \cc{0.22}         & \cc{-}               & \cc{-}                     & \cc{-}          \\
%             ChatGPT-4o (7)              & 0.24              & -                    & -                           & -           \\
%             \Xhline{2\arrayrulewidth}
%             \cc{\textbf{Average}}           &\cc{0.24}          & \cc{-}               & \cc{\textbf{-}}                &  \cc{ }           \\
%             \Xhline{2\arrayrulewidth}
%             \end{tabular}
% \end{minipage}
% \end{table*}
